The Statistical Relationship between White-light Emission and Photospheric Magnetic Field Changes in Flares

Continuum emission, also called white-light emission (WLE), and permanent changes of the magnetic field ($\Delta{B}_{{\rm{LOS}}}$) are often observed during solar flares. But their relation and their precise mechanisms are still unknown. We study statistically the relationship between $\Delta{B}_{{\rm{LOS}}}$ and WLE during 75 solar flares of different strengths and locations on the solar disk. We analyze SDO/HMI data and determine for each pixel in each flare if it exhibited WLE and/or $\Delta{B}_{{\rm{LOS}}}$. We then investigate the occurrence, strength, and spatial size of the WLE, its dependence on flare energy, and its correlation to the occurrence of $\Delta{B}_{{\rm{LOS}}}$. We detected WLE in 44/75 flares and $\Delta{B}_{{\rm{LOS}}}$ in 59/75 flares. We find that WLE and $\Delta{B}_{{\rm{LOS}}}$ are related, and their locations often overlap between 0-60\%. Not all locations coincide, thus potentially indicating differences in their origin. We find that the WL area is related to the flare class by a power law and extend the findings of previous studies, that the WLE is related to the flare class by a power law, to also be valid for C-class flares. To compare unresolved (Sun-as-a-star) WL measurements to our data, we derive a method to calculate temperatures and areas of such data under the black-body assumption. The calculated unresolved WLE areas improve, but still differ to the resolved flaring area by about a factor of 5-10 (previously 10-20), which could be explained by various physical or instrumental causes. This method could also be applied to stellar flares to determine their temperatures and areas independently.

==> flare_sample.tex <==
\startlongtable
\begin{deluxetable*}{rlccccccccc}
%\tabletypesize{\small }
%\tablecolumns{11} 
\tablewidth{0pt}
\tablecaption{List of flares\label{tab_sample}} 
\tablehead{
&\colhead{Observation}              & \colhead{GOES} & 
\colhead{GOES}         & \colhead{NOAA}   & \colhead{Latitude} & \colhead{Longitude} & \colhead{${\rm A}_{\BLOS{}}$}& \colhead{${\rm F}_{|\BLOS{}|}$}   & \colhead{${\rm A}_{\rm WL}$} & \colhead{${\rm F}_{\rm WL}$}\\
\colhead{Index}&\colhead{date} & \colhead{Peak} & \colhead{Class} & \colhead{AR}   & \colhead{(deg)}  & \colhead{(deg)} & \colhead{(Mm$^2$)} & \colhead{(Mx)} & \colhead{(Mm$^2$)} & \colhead{(W m$^{-2}$)}}
%\decimalcolnumbers
\startdata
\textbf{\texttt{FL}01} & 2011 Aug 9  & 08:05 &  X6.9  & 11263 &  14.9 N  &  69.6 W  & 367.8 & 6.1E+23 & 341.8 & 6.8E-2\\
\textbf{\texttt{FL}02} & 2014 Feb 25  & 00:49 &  X4.9  & 11990 &  12.0 S  &  81.9 E  & 596.4 & 1.0E+24 & 822.2 & 1.2E-1\\
\textbf{\texttt{FL}03} & 2014 Oct 24  & 21:41 &  X3.1  & 12192 &  11.1 S  &  20.5 W  & 295.5 & 8.5E+23 & 515.2 & 4.9E-2\\
\textbf{\texttt{FL}04} & 2014 Jun 10  & 11:42 &  X2.2  & 12087 &  15.0 S  &  79.8 E  & 105.7 & 3.9E+22 & 164.2 & 3.6E-2\\
\textbf{\texttt{FL}05} & 2011 Feb 15  & 01:56 &  X2.2  & 11158 &  20.9 S  &  10.8 W  & 187.2 & 4.0E+23 & 79.2 & 8.2E-3\\
\textbf{\texttt{FL}06} & 2015 Mar 11  & 16:22 &  X2.1  & 12297 &  17.0 S  &  21.0 E  & 56.9 & 2.9E+22 & 91.2 & 1.1E-2\\
\textbf{\texttt{FL}07} & 2014 Oct 27  & 14:47 &  X2.0  & 12192 &  18.8 S  &  57.4 W  & 71.7 & 3.9E+22 & 313.1 & 2.0E-2\\
\textbf{\texttt{FL}08} & 2011 Sep 24  & 09:39 &  X1.9  & 11302 &  12.0 N  &  59.9 E  & 295.7 & 5.3E+23 & 626.1 & 3.3E-2\\
\textbf{\texttt{FL}09} & 2014 Dec 20  & 00:28 &  X1.8  & 12242 &  19.1 S  &  29.0 W  & 194.5 & 3.7E+23 & 128.6 & 9.7E-3\\
\textbf{\texttt{FL}10} & 2012 Oct 23  & 03:17 &  X1.8  & 11598 &  13.3 S  &  58.9 E  & 327.3 & 8.6E+23 & 178.0 & 3.7E-2\\
\textbf{\texttt{FL}11} & 2014 Oct 22  & 14:28 &  X1.6  & 12192 &  14.4 S  &  13.9 E  & 132.9 & 2.0E+23 & 276.2 & 2.4E-2\\
\textbf{\texttt{FL}12} & 2014 Jun 10  & 12:52 &  X1.5  & 12087 &  17.0 S  &  81.9 E  & 71.4 & 8.1E+21 & 100.6 & 2.0E-3\\
\textbf{\texttt{FL}13} & 2011 Mar 9  & 23:23 &  X1.5  & 11166 &  08.0 N  &  11.8 W  & 76.0 & 7.0E+22 & 24.4 & 2.0E-3\\
\textbf{\texttt{FL}14} & 2012 Jul 12  & 16:50 &  X1.4  & 11520 &  14.0 S  &  03.9 W  & 140.9 & 2.3E+23 &  \nodata &  \nodata\\
\textbf{\texttt{FL}15} & 2013 Nov 10  & 05:14 &  X1.1  & 11890 &  13.4 S  &  13.9 W  & 102.9 & 1.4E+23 & 55.3 & 1.3E-2\\
\textbf{\texttt{FL}16} & 2014 Jun 11  & 09:06 &  X1.0  & 12087 &  18.0 S  &  64.9 E  & 107.0 & 6.2E+22 & 81.0 & 1.1E-2\\
\textbf{\texttt{FL}17} & 2014 Mar 29  & 17:48 &  X1.0  & 12017 &  10.2 N  &  32.9 W  & 86.5 & 7.6E+22 & 66.2 & 5.8E-3\\
\textbf{\texttt{FL}18} & 2013 Oct 28  & 02:03 &  X1.0  & 11875 &  04.0 N  &  66.0 W  & 153.5 & 9.4E+22 & 100.8 & 3.8E-3\\
\textbf{\texttt{FL}19} & 2011 Jul 30  & 02:09 &  M9.3  & 11261 &  14.0 N  &  34.9 E  & 109.0 & 1.6E+23 & 68.2 & 1.5E-2\\
\textbf{\texttt{FL}20} & 2011 Sep 8  & 15:46 &  M6.7  & 11283 &  14.0 N  &  39.9 W  & 56.1 & 2.8E+22 & 32.8 & 2.6E-3\\
\textbf{\texttt{FL}21} & 2011 Feb 18  & 10:11 &  M6.6  & 11158 &  21.1 S  &  55.0 W  & 131.4 & 1.6E+23 & 64.6 & 1.2E-2\\
\textbf{\texttt{FL}22} & 2011 Feb 13  & 17:38 &  M6.6  & 11158 &  19.9 S  &  03.9 E  & 106.6 & 1.7E+23 & 33.5 & 3.2E-3\\
\textbf{\texttt{FL}23} & 2013 Dec 31  & 21:58 &  M6.4  & 11936 &  15.5 S  &  36.0 W  & 97.0 & 8.1E+22 &  \nodata &  \nodata\\
\textbf{\texttt{FL}24} & 2012 Mar 9  & 03:53 &  M6.3  & 11429 &  15.8 N  &  03.4 W  & 53.8 & 3.2E+22 &  \nodata &  \nodata\\
\textbf{\texttt{FL}25} & 2012 Jul 5  & 11:44 &  M6.1  & 11515 &  18.7 S  &  32.6 W  & 89.4 & 7.6E+22 & 82.9 & 9.0E-3\\
\textbf{\texttt{FL}26} & 2011 Sep 24  & 20:36 &  M5.8  & 11302 &  13.0 N  &  52.0 E  & 46.2 & 2.8E+22 & 49.5 & 6.2E-3\\
\textbf{\texttt{FL}27} & 2012 May 10  & 04:18 &  M5.7  & 11476 &  12.9 N  &  22.0 E  & 91.0 & 9.5E+22 & 44.6 & 4.0E-3\\
\textbf{\texttt{FL}28} & 2012 Jul 4  & 09:55 &  M5.3  & 11515 &  17.3 S  &  18.0 W  & 72.6 & 6.9E+22 & 46.3 & 7.5E-3\\
\textbf{\texttt{FL}29} & 2014 Feb 4  & 04:00 &  M5.2  & 11967 &  12.9 S  &  06.9 W  & 59.8 & 5.2E+22 & 50.2 & 3.2E-3\\
\textbf{\texttt{FL}30} & 2012 Jul 5  & 03:36 &  M4.7  & 11515 &  18.3 S  &  29.2 W  & 58.6 & 4.4E+22 & 52.2 & 1.0E-2\\
\textbf{\texttt{FL}31} & 2011 Mar 14  & 19:52 &  M4.2  & 11169 &  16.1 N  &  49.6 W  & 102.7 & 8.6E+22 & 43.6 & 2.8E-3\\
\textbf{\texttt{FL}32} & 2014 Oct 24  & 07:48 &  M4.0  & 12192 &  20.7 S  &  07.3 W  & 74.0 & 5.9E+22 &  \nodata &  \nodata\\
\textbf{\texttt{FL}33} & 2011 Oct 2  & 00:50 &  M3.9  & 11305 &  09.0 N  &  12.0 W  & 29.5 & 1.1E+22 &  \nodata &  \nodata\\
\textbf{\texttt{FL}34} & 2011 Sep 24  & 17:25 &  M3.1  & 11302 &  13.0 N  &  54.0 E  & 29.4 & 5.5E+21 & 16.0 & 5.2E-4\\
\textbf{\texttt{FL}35} & 2011 Sep 24  & 19:21 &  M3.0  & 11302 &  12.7 N  &  42.7 E  & 28.9 & 5.6E+21 &  \nodata &  \nodata\\
\textbf{\texttt{FL}36} & 2010 Oct 16  & 19:12 &  M2.9  & 11112 &  20.8 S  &  27.9 W  & 79.8 & 8.0E+22 & 9.5 & 2.0E-3\\
\textbf{\texttt{FL}37} & 2011 Sep 9  & 06:09 &  M2.7  & 11283 &  16.0 N  &  47.0 W  & 67.3 & 3.6E+22 & 9.9 & 6.8E-4\\
\textbf{\texttt{FL}38} & 2011 Dec 31  & 13:15 &  M2.4  & 11389 &  25.9 S  &  46.0 E  & 52.3 & 2.3E+22 & 19.2 & 2.4E-3\\
\textbf{\texttt{FL}39} & 2012 Jun 29  & 09:20 &  M2.2  & 11513 &  17.0 N  &  36.9 E  & 39.0 & 1.5E+22 & 10.5 & 8.3E-4\\
\textbf{\texttt{FL}40} & 2011 Dec 29  & 13:50 &  M1.9  & 11389 &  25.2 S  &  70.7 E  & 47.4 & 7.7E+21 &  \nodata &  \nodata\\
\textbf{\texttt{FL}41} & 2012 Jun 9  & 16:53 &  M1.8  & 11504 &  17.0 S  &  73.9 E  & 62.0 & 1.1E+22 & 30.6 & 8.2E-4\\
\textbf{\texttt{FL}42} & 2012 Jun 30  & 18:32 &  M1.6  & 11513 &  13.9 N  &  18.0 E  & 18.3 & 4.3E+21 &  \nodata &  \nodata\\
\textbf{\texttt{FL}43} & 2012 Jul 6  & 08:23 &  M1.5  & 11515 &  17.0 S  &  39.9 W  & 113.3 & 9.1E+22 & 11.6 & 7.2E-4\\
\textbf{\texttt{FL}44} & 2011 Dec 31  & 16:26 &  M1.5  & 11389 &  25.7 S  &  42.7 E  & 47.9 & 1.7E+22 & 6.3 & 6.6E-4\\
\textbf{\texttt{FL}45} & 2011 Dec 26  & 02:27 &  M1.5  & 11387 &  21.0 S  &  32.9 W  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}46} & 2012 May 8  & 13:08 &  M1.4  & 11476 &  12.9 N  &  44.0 E  & 52.2 & 2.4E+22 & 16.5 & 9.6E-4\\
\textbf{\texttt{FL}47} & 2011 Feb 18  & 13:03 &  M1.4  & 11158 &  21.1 S  &  55.8 W  & 69.7 & 3.2E+22 & 30.4 & 1.0E-3\\
\textbf{\texttt{FL}48} & 2012 Jul 4  & 14:40 &  M1.3  & 11515 &  18.0 S  &  18.0 W  & 43.0 & 2.2E+22 & 12.5 & 1.0E-3\\
\textbf{\texttt{FL}49} & 2012 May 5  & 23:01 &  M1.3  & 11476 &  08.9 N  &  74.7 E  & 19.1 & 9.9E+20 & 15.8 & 4.8E-4\\
\textbf{\texttt{FL}50} & 2012 Mar 17  & 20:39 &  M1.3  & 11434 &  20.0 S  &  25.0 W  & 16.0 & 2.9E+21 &  \nodata &  \nodata\\
\textbf{\texttt{FL}51} & 2011 Feb 18  & 21:04 &  M1.3  & 11162 &  18.1 N  &  03.7 W  & 60.2 & 4.4E+22 &  \nodata &  \nodata\\
\textbf{\texttt{FL}52} & 2012 May 6  & 01:18 &  M1.1  & 11476 &  11.0 N  &  72.9 E  & 31.6 & 2.9E+21 & 49.3 & 2.3E-3\\
\textbf{\texttt{FL}53} & 2011 Nov 5  & 11:21 &  M1.1  & 11339 &  19.7 N  &  41.1 E  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}54} & 2011 Sep 22  & 10:00 &  M1.1  & 11295 &  25.1 N  &  57.2 W  & 36.7 & 7.8E+21 &  \nodata &  \nodata\\
\textbf{\texttt{FL}55} & 2012 Apr 27  & 08:24 &  M1.0  & 11466 &  13.0 N  &  29.5 W  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}56} & 2011 Mar 15  & 00:22 &  M1.0  & 11169 &  11.8 N  &  83.3 W  & 39.7 & 1.2E+22 & 12.7 & 5.8E-4\\
\textbf{\texttt{FL}57} & 2012 Jul 3  & 03:42 &  C9.9  & 11515 &  18.2 S  &  02.4 W  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}58} & 2011 Aug 3  & 07:58 &  C8.7  & 11261 &  15.8 N  &  29.3 W  & 41.0 & 1.9E+22 &  \nodata &  \nodata\\
\textbf{\texttt{FL}59} & 2011 Aug 8  & 22:09 &  C7.7  & 11263 &  17.4 N  &  66.5 W  & 48.2 & 1.2E+22 & 21.6 & 4.6E-4\\
\textbf{\texttt{FL}60} & 2011 May 27  & 16:43 &  C5.6  & 11226 &  21.4 S  &  89.8 E  &  \nodata &  \nodata & 10.8 & 6.5E-5\\
\textbf{\texttt{FL}61} & 2011 Oct 20  & 15:39 &  C5.4  & 11324 &  11.5 N  &  47.8 E  & 38.0 & 1.0E+22 &  \nodata &  \nodata\\
\textbf{\texttt{FL}62} & 2011 Dec 5  & 15:18 &  C4.9  & 11363 &  20.3 S  &  02.4 W  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}63} & 2011 Nov 22  & 04:04 &  C4.7  & 11356 &  12.7 N  &  50.2 E  & 3.5 & 7.8E+19 &  \nodata &  \nodata\\
\textbf{\texttt{FL}64} & 2011 Dec 21  & 04:55 &  C4.3  & 11382 &  19.4 S  &  02.1 E  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}65} & 2011 Nov 7  & 03:10 &  C3.5  & 11339 &  20.3 N  &  22.0 E  & 41.1 & 1.7E+22 &  \nodata &  \nodata\\
\textbf{\texttt{FL}66} & 2011 Jul 27  & 10:02 &  C3.0  & 11260 &  18.6 N  &  40.6 E  & 23.0 & 4.6E+21 &  \nodata &  \nodata\\
\textbf{\texttt{FL}67} & 2011 Aug 20  & 22:58 &  C2.9  & 11271 &  13.6 N  &  12.0 E  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}68} & 2011 Oct 27  & 18:44 &  C2.6  & 11333 &  15.0 N  &  13.5 E  &  \nodata &  \nodata &  \nodata &  \nodata\\
\tablenotemark{a}\textbf{\texttt{FL}69} & 2011 Mar 31  & 15:35 &  C2.6  & 11176 &  16.0 S  &  39.8 W  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}70} & 2011 Sep 3  & 07:56 &  C2.4  & 11281 &  21.0 S  &  01.1 W  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}71} & 2011 Apr 23  & 07:34 &  C2.4  & 11195 &  16.0 S  &  23.8 E  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}72} & 2011 Aug 1  & 12:40 &  C2.0  & 11261 &  18.2 N  &  01.8 W  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}73} & 2011 Apr 12  & 03:46 &  C1.7  & 11190 &  11.7 N  &  25.0 E  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}74} & 2011 Apr 18  & 19:02 &  C1.5  & 11193 &  16.4 N  &  11.7 E  &  \nodata &  \nodata &  \nodata &  \nodata\\
\textbf{\texttt{FL}75} & 2011 Jul 16  & 17:05 &  B6.2  & 11254 &  24.3 S  &  42.8 E  &  \nodata &  \nodata &  \nodata &  \nodata\\
\enddata
\tablenotetext{a}{$\textbf{\texttt{FL}69}$ was excluded from the analysis because it has gaps in the data.}
\tablecomments{The details of the flares are shown in columns 1 - 7. The areas, and fluxes of \blos{} and WL emission are in columns 8 - 11.}
\end{deluxetable*}
